ezBFT: Decentralizing Byzantine Fault-Tolerant State Machine Replication

We present ezBFT, a novel leaderless, distributed consensus protocol capable of tolerating byzantine faults. ezBFT's main goal is to minimize the client-side latency in WAN deployments. It achieves this by (i) having no designated primary replica, and instead, enabling every replica to order the requests that it receives from clients; (ii) using only three communication steps to order requests in the common case; and (iii) involving clients actively in the consensus process. In addition, ezBFT minimizes the potentially negative effect of a byzantine replica on the overall system performance. We developed ezBFT's formal specification in TLA+, show that it provides the classic properties of BFT protocols including consistency, stability, and liveness, and developed an implementation. Our experimental evaluation reveals that ezBFT improves client-side latency by as much as 40% over state-of-the-art byzantine fault-tolerant protocols including PBFT, FaB, and Zyzzyva.

==> motivation.tex <==



